A Bayesian approach to calibrating hydrogen flame kinetics using many experiments and parameters

First-principles Markov Chain Monte Carlo sampling is used to investigate uncertainty quantification and uncertainty propagation in parameters describing hydrogen kinetics. Specifically, we sample the posterior distribution of thirty-one parameters focusing on the H2O2 and HO2 reactions resulting from conditioning on ninety-one experiments. Established literature values are used for the remaining parameters in the mechanism. The samples are computed using an affine invariant sampler starting with broad, noninformative priors. Autocorrelation analysis shows that O(1M) samples are sufficient to obtain a reasonable sampling of the posterior. The resulting distribution identifies strong positive and negative correlations and several non-Gaussian characteristics. Using samples drawn from the posterior, we investigate the impact of parameter uncertainty on the prediction of two more complex flames: a 2D premixed flame kernel and the ignition of a hydrogen jet issuing into a heated chamber. The former represents a combustion regime similar to the target experiments used to calibrate the mechanism and the latter represents a different combustion regime. For the premixed flame, the net amount of product after a given time interval has a standard deviation of less than 2% whereas the standard deviation of the ignition time for the jet is more than 10%. The samples used for these studies are posted online. These results indicate the degree to which parameters consistent with the target experiments constrain predicted behavior in different combustion regimes. This process provides a framework for both identifying reactions for further study from candidate mechanisms as well as combining uncertainty quantification and propagation to, ultimately, tie uncertainty in laboratory flame experiments to uncertainty in end-use numerical predictions of more complicated scenarios.

==> expts.tex <==
\begin{tabular}{lllrrrrrrrrr}
\toprule
{} & Bath &         Ref &     T0 &  Target &     Tf &  XH2 &  XHE &  XO2 &   p0 &  phi &  sigma \\
\midrule
ID            &      &             &        &         &        &      &      &      &      &      &        \\
BurkeCDJ10\_0  &  NaN &  BurkeCDJ10 &  295.0 &    95.3 & 1600.0 &  0.1 &  0.8 &  0.1 &  1.0 &  0.9 &   10.4 \\
BurkeCDJ10\_1  &  NaN &  BurkeCDJ10 &  295.0 &    77.4 & 1600.0 &  0.1 &  0.8 &  0.1 &  5.0 &  0.9 &   12.8 \\
BurkeCDJ10\_2  &  NaN &  BurkeCDJ10 &  295.0 &    45.9 & 1600.0 &  0.1 &  0.8 &  0.1 & 10.0 &  0.9 &    4.9 \\
BurkeCDJ10\_3  &  NaN &  BurkeCDJ10 &  295.0 &    28.3 & 1600.0 &  0.1 &  0.8 &  0.1 & 15.0 &  0.9 &    2.5 \\
BurkeCDJ10\_4  &  NaN &  BurkeCDJ10 &  295.0 &    20.0 & 1600.0 &  0.1 &  0.8 &  0.1 & 20.0 &  0.9 &    1.6 \\
BurkeCDJ10\_5  &  NaN &  BurkeCDJ10 &  295.0 &    15.2 & 1600.0 &  0.1 &  0.8 &  0.1 & 25.0 &  0.9 &    1.2 \\
BurkeCDJ10\_6  &  NaN &  BurkeCDJ10 &  295.0 &    83.0 & 1500.0 &  0.1 &  0.8 &  0.1 &  1.0 &  1.0 &   13.8 \\
BurkeCDJ10\_7  &  NaN &  BurkeCDJ10 &  295.0 &    48.7 & 1500.0 &  0.1 &  0.8 &  0.1 &  5.0 &  1.0 &    9.2 \\
BurkeCDJ10\_8  &  NaN &  BurkeCDJ10 &  295.0 &    27.3 & 1500.0 &  0.1 &  0.8 &  0.1 & 10.0 &  1.0 &    3.6 \\
BurkeCDJ10\_9  &  NaN &  BurkeCDJ10 &  295.0 &    87.0 & 1600.0 &  0.1 &  0.8 &  0.1 &  1.0 &  1.0 &    9.2 \\
BurkeCDJ10\_10 &  NaN &  BurkeCDJ10 &  295.0 &    61.9 & 1600.0 &  0.1 &  0.8 &  0.1 &  5.0 &  1.0 &   10.8 \\
BurkeCDJ10\_11 &  NaN &  BurkeCDJ10 &  295.0 &    40.7 & 1600.0 &  0.1 &  0.8 &  0.1 & 10.0 &  1.0 &    4.5 \\
BurkeCDJ10\_12 &  NaN &  BurkeCDJ10 &  295.0 &    28.7 & 1600.0 &  0.1 &  0.8 &  0.1 & 15.0 &  1.0 &    2.7 \\
BurkeCDJ10\_13 &  NaN &  BurkeCDJ10 &  295.0 &    21.4 & 1600.0 &  0.1 &  0.8 &  0.1 & 20.0 &  1.0 &    1.8 \\
BurkeCDJ10\_14 &  NaN &  BurkeCDJ10 &  295.0 &    14.5 & 1600.0 &  0.1 &  0.8 &  0.1 & 25.0 &  1.0 &    1.1 \\
BurkeDJ11\_5   &  NaN &   BurkeDJ11 &  295.0 &    61.0 & 1400.0 &  0.1 &  0.8 &  0.1 &  1.0 &  0.5 &    3.6 \\
BurkeDJ11\_6   &  NaN &   BurkeDJ11 &  295.0 &    37.9 & 1400.0 &  0.1 &  0.8 &  0.1 &  2.5 &  0.5 &    4.4 \\
BurkeDJ11\_7   &  NaN &   BurkeDJ11 &  295.0 &    23.1 & 1400.0 &  0.1 &  0.8 &  0.1 &  5.0 &  0.5 &    2.2 \\
BurkeDJ11\_8   &  NaN &   BurkeDJ11 &  295.0 &    15.0 & 1400.0 &  0.1 &  0.8 &  0.1 &  7.5 &  0.5 &    1.5 \\
BurkeDJ11\_9   &  NaN &   BurkeDJ11 &  295.0 &     8.2 & 1400.0 &  0.1 &  0.8 &  0.1 & 10.0 &  0.5 &    0.7 \\
BurkeDJ11\_10  &  NaN &   BurkeDJ11 &  295.0 &   105.1 & 1600.0 &  0.1 &  0.8 &  0.1 &  1.0 &  0.5 &    3.4 \\
BurkeDJ11\_11  &  NaN &   BurkeDJ11 &  295.0 &    64.3 & 1600.0 &  0.1 &  0.8 &  0.1 &  5.0 &  0.5 &    2.7 \\
BurkeDJ11\_12  &  NaN &   BurkeDJ11 &  295.0 &    40.1 & 1600.0 &  0.1 &  0.8 &  0.1 & 10.0 &  0.5 &    1.7 \\
BurkeDJ11\_13  &  NaN &   BurkeDJ11 &  295.0 &    59.7 & 1400.0 &  0.1 &  0.8 &  0.1 &  1.0 &  0.7 &    4.3 \\
BurkeDJ11\_14  &  NaN &   BurkeDJ11 &  295.0 &    42.3 & 1400.0 &  0.1 &  0.8 &  0.1 &  2.5 &  0.7 &    3.4 \\
BurkeDJ11\_15  &  NaN &   BurkeDJ11 &  295.0 &    27.6 & 1400.0 &  0.1 &  0.8 &  0.1 &  5.0 &  0.7 &    1.7 \\
BurkeDJ11\_16  &  NaN &   BurkeDJ11 &  295.0 &    17.7 & 1400.0 &  0.1 &  0.8 &  0.1 &  7.5 &  0.7 &    1.1 \\
BurkeDJ11\_17  &  NaN &   BurkeDJ11 &  295.0 &    10.3 & 1400.0 &  0.1 &  0.8 &  0.1 & 10.0 &  0.7 &    0.8 \\
BurkeDJ11\_18  &  NaN &   BurkeDJ11 &  295.0 &    97.7 & 1600.0 &  0.1 &  0.8 &  0.1 &  1.0 &  0.7 &    3.9 \\
BurkeDJ11\_19  &  NaN &   BurkeDJ11 &  295.0 &    67.0 & 1600.0 &  0.1 &  0.8 &  0.1 &  5.0 &  0.7 &    3.2 \\
BurkeDJ11\_20  &  NaN &   BurkeDJ11 &  295.0 &    44.3 & 1600.0 &  0.1 &  0.8 &  0.1 & 10.0 &  0.7 &    2.0 \\
BurkeDJ11\_21  &  NaN &   BurkeDJ11 &  295.0 &    31.4 & 1600.0 &  0.1 &  0.8 &  0.1 & 15.0 &  0.7 &    2.1 \\
BurkeDJ11\_22  &  NaN &   BurkeDJ11 &  295.0 &    22.4 & 1600.0 &  0.1 &  0.8 &  0.1 & 20.0 &  0.7 &    1.4 \\
BurkeDJ11\_23  &  NaN &   BurkeDJ11 &  295.0 &    16.3 & 1600.0 &  0.1 &  0.8 &  0.1 & 25.0 &  0.7 &    1.9 \\
BurkeDJ11\_33  &  NaN &   BurkeDJ11 &  295.0 &    95.3 & 1600.0 &  0.1 &  0.8 &  0.1 &  1.0 &  0.9 &   12.4 \\
BurkeDJ11\_34  &  NaN &   BurkeDJ11 &  295.0 &    66.2 & 1600.0 &  0.1 &  0.8 &  0.1 &  5.0 &  0.9 &    3.4 \\
BurkeDJ11\_35  &  NaN &   BurkeDJ11 &  295.0 &    87.0 & 1600.0 &  0.1 &  0.8 &  0.1 &  1.0 &  1.0 &    9.2 \\
BurkeDJ11\_36  &  NaN &   BurkeDJ11 &  295.0 &    61.9 & 1600.0 &  0.1 &  0.8 &  0.1 &  5.0 &  1.0 &   10.8 \\
BurkeDJ11\_37  &  NaN &   BurkeDJ11 &  295.0 &    40.7 & 1600.0 &  0.1 &  0.8 &  0.1 & 10.0 &  1.0 &    4.5 \\
fls1a         &   N2 &     [27–31] &  298.2 &   204.0 &    nan & 29.6 &  0.0 & 14.8 &  1.0 &  1.0 &   20.0 \\
fls2a         &   He &        [27] &  298.2 &   206.0 &    nan & 20.0 &  0.0 & 10.0 &  1.0 &  1.0 &   20.0 \\
fls3a         &   He &        [27] &  298.2 &    58.0 &    nan & 13.8 &  0.0 &  6.9 & 15.0 &  1.0 &    6.0 \\
flw1a         &   N2 &        [13] &  914.0 &     8.6 &    nan &  1.2 &  0.0 &  0.6 & 15.7 &  1.0 &    0.5 \\
flw2a         &   N2 &        [13] &  935.0 &    13.0 &    nan &  1.0 &  0.0 &  0.5 &  6.0 &  1.0 &    0.5 \\
flw3a         &   N2 &        [13] &  943.0 &    98.0 &    nan &  1.0 &  0.0 &  1.5 &  2.5 &  0.3 &   10.0 \\
flw4a         &   N2 &        [13] &  880.0 &   261.0 &    nan &  0.5 &  0.0 &  0.5 &  0.3 &  0.5 &   20.0 \\
flw8a         &   N2 &        [13] &  934.0 &    19.0 &    nan &  0.9 &  0.0 &  0.5 &  3.0 &  1.0 &    1.0 \\
flw8b         &   N2 &        [13] &  934.0 &    70.0 &    nan &  0.9 &  0.0 &  0.5 &  3.0 &  1.0 &    5.0 \\
ign2a         &   Ar &        [37] & 1033.0 &   238.0 &    nan & 20.0 &  0.0 & 10.0 &  0.5 &  1.0 &  140.0 \\
ign2b         &   Ar &        [37] & 1510.0 &    29.0 &    nan & 20.0 &  0.0 & 10.0 &  0.5 &  1.0 &   20.0 \\
ign3a         &   Ar &        [38] & 1754.0 &    10.0 &    nan &  0.5 &  0.0 &  0.2 & 33.0 &  1.0 &    3.0 \\
ign4a         &   Ar &        [38] & 1189.0 &   293.0 &    nan &  2.0 &  0.0 &  1.0 & 33.0 &  1.0 &  100.0 \\
ign4b         &   Ar &        [38] & 1300.0 &    11.0 &    nan &  2.0 &  0.0 &  1.0 & 33.0 &  1.0 &    4.0 \\
ign5a         &   Ar &        [38] & 1524.0 &    54.0 &    nan &  0.1 &  0.0 &  0.1 & 64.0 &  1.0 &   25.0 \\
\bottomrule
\end{tabular}

